Large Vocabulary Automatic Chord Estimation Using Deep Neural Nets: Design Framework, System Variations and Limitations

In this paper, we propose a new system design framework for large vocabulary automatic chord estimation. Our approach is based on an integration of traditional sequence segmentation processes and deep learning chord classification techniques. We systematically explore the design space of the proposed framework for a range of parameters, namely deep neural nets, network configurations, input feature representations, segment tiling schemes, and training data sizes. Experimental results show that among the three proposed deep neural nets and a baseline model, the recurrent neural network based system has the best average chord quality accuracy that significantly outperforms the other considered models. Furthermore, our bias-variance analysis has identified a glass ceiling as a potential hindrance to future improvements of large vocabulary automatic chord estimation systems.

==> figs/old/figures.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                               %%
%% Figures                       %%
%%                               %%
%% NB: this is for captions and  %%
%% Titles. All graphics must be  %%
%% submitted separately and NOT  %%
%% included in the Tex document  %%
%%                               %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%
%% Do not use \listoffigures as most will included as separate files

\section*{Figures}
\begin{figure}
	%\centering
	%\includegraphics {figs/1-inversions.pdf}
	\caption{Four chord progressions that contain bass line continuations which require chord inversions (those with a ``/'' mark). In all these sequences, the basses are either walking downward or upward. Progressions like 1, 2 and 3 are very popular among pop/rock. Progression 4 induces a key shift from C \textit{major} to F\# \textit{minor}.}
	\label{fig:wdwu}
\end{figure}

\begin{figure}
	%\centering
	%\includegraphics {figs/2-sys.pdf}
	\caption{The LVACE system framework. As for training, each data sample first goes through a feature extraction process, then it is segmented by ground truth labels. After segment tiling, it is used to train a deep neural nets. The validation process shares the same modules with training, except for segmentation, where a GMM-HMM method is applied.}
	\label{fig:sysover}
\end{figure}

\begin{figure}
	%\centering
	%\includegraphics{figs/3-btp.pdf}
	\caption{The bass (+) and treble (.) profiles. They are both computed in the shape of Rayleigh distributions with scale parameters 16.8 (for bass) and 42 (for treble) respectively. The horizontal axis stands for MIDI pitch numbers. The vertical axis represents normalized profile amplitudes from 0 to 1.}
	\label{fig:btprofile}
\end{figure}

\begin{figure}
	%\centering
	%\includegraphics{figs/4-rnn.pdf}
	\caption{The bidirectional recurrent neural network architecture used in our system. Both hidden layers employ LSTM units in place of normal logistic units. The RNN is expanded to $N$ frames, with mean pooling to summarize results.}
	\label{fig:brnn}
\end{figure}

\begin{figure}
	%\centering
	%\includegraphics{figs/5-lstm.pdf}
	\caption{The structure of a long short-term memory unit}
	\label{fig:lstm}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/6-ch-configs.pdf}
	\caption{Exploring different network configurations at -ch level. All models are trained with JKU-6seg-ch.}
	\label{fig:ch-configs}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/7-ns-configs.pdf}
	\caption{Exploring different network configurations at -ns level. All models are trained with JKU-6seg-ns.}
	\label{fig:ns-configs}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/8-ch-nseg.pdf}
	\caption{Exploring effect of segment tiling at -ch level. All models are trained with JKU-ch-[800*2]}
	\label{fig:ch-nseg}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/9-ns-nseg.pdf}
	\caption{Exploring effect of segment tiling at -ns level. All models are trained with JKU-ns-[800*2]}
	\label{fig:ns-nseg}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/10-ch-data.pdf}
	\caption{Exploring different training data size at -ch level. All models are trained with 6seg-ch-[800*2].}
	\label{fig:ch-data}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/11-ns-data.pdf}
	\caption{Exploring training data size at -ns level. All models are trained with 6seg-ns-[800*2].}
	\label{fig:ns-data}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/12-av\_skewed.pdf}
	\caption{Performance on common and skewed chords in different neural nets. All models are trained with 6seg-[800*2].}
	\label{fig:skewed}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/13-av\_acqa.pdf}
	\caption{Average ACQAs of \textit{SeventhsBass} Vocabulary. All models are trained with 6seg-[800*2].}
	\label{fig:acqa}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/14-ftestacqa.eps}
	\caption{Friedman test with Tukey HSD: ACQAs of different system variants}
	\label{fig:friedmanacqa}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/15-ftestwcsr.eps}
	\caption{Friedman test with Tukey HSD: WCSRs of different system variants}
	\label{fig:friedmanwcsr}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/16-cp\_wcsr.pdf}
	\caption{Compare system representatives with Chordino on WCSRs. All models are trained with JKURB-6seg-ns-[800*2].}
	\label{fig:compchordino}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/17-cp\_acqa.pdf}
	\caption{Compare system representatives with Chordino on ACQAs. All models are trained with JKURB-6seg-ns-[800*2].}
	\label{fig:acqachordino}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/18-ftestwcsrbl.eps}
	\caption{Friedman test with Tukey HSD: WCSRs compared with the baseline}
	\label{fig:friedmanwcsrbl}
\end{figure}

\begin{figure}
	\centering
	\includegraphics{figs/19-ftestacqabl.eps}
	\caption{Friedman test with Tukey HSD: ACQAs compared with the baseline}
	\label{fig:friedmanacqabl}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                               %%
%% Tables                        %%
%%                               %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Use of \listoftables is discouraged.
%%

\section*{Tables}
%\begin{table}[h!]
%\caption{Sample table title. This is where the description of the table should go.}
%      \begin{tabular}{cccc}
%        \hline
%           & B1  &B2   & B3\\ \hline
%        A1 & 0.1 & 0.2 & 0.3\\
%        A2 & ... & ..  & .\\
%        A3 & ..  & .   & .\\ \hline
%      \end{tabular}
%\end{table}

\begin{table}
	\caption{GMM-HMM segmentation settings. Different parameters are assigned to different note degree within a chord.}
	\centering
	\footnotesize
	\begin{tabular}{|c|c|c|} \hline
		& $\mu$ & $\sigma^2$ \\ \hline
		Bass - chord bass & 1 & 0.1 \\ \hline
		Bass - not chord bass and is chord note & 1 & 0.5  \\ \hline
		Bass - neither chord bass nor chord note & 0 & 0.1 \\ \hline
		Treble - chord note & 1 & 0.2  \\ \hline
		Treble - not chord note & 0 & 0.2 \\ \hline
		No Chord (for all notes)  & 1 & 0.2  \\ \hline
	\end{tabular}
	\label{tab:gaussian}
\end{table}

\begin{table}
	\caption{Variations considered in this study}
	\centering
	\footnotesize
	\begin{tabular}{|c|c|c|} \hline
		Dimension & Variation \\ \hline
		neural net architecture & FCNN; DBN; BLSTM-RNN \\ \hline
		segment tiling & 1; 2; 3; 6; 9; 12 (seg) \\ \hline
		layer depth & 2; 3; 4 \\ \hline
		layer width & 500; 800; 1000 \\ \hline
		input representation & notegram (-ns); chromagram (-ch) \\ \hline
		training data size & JK; JKU; JKUR; JKURB \\ \hline
	\end{tabular}
	\label{tab:varexplore}
\end{table}



==> figs/pdfplot.tex <==
\subsection{Network configurations} \label{sec:3-p2}

\Hsection{-ch level}

\pgfplotsset{width=8cm,height=4cm,every node near coord/.append style={font=\scriptsize}}
\begin{figure}[htb]
	\centering
	\begin{tikzpicture}
	\begin{axis}[
	title={FCNN-JKU-6seg-ch SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={[500*2],[500*3],[500*4],[800*2],[800*3],[800*4],[1000*2],[1000*3],[1000*4]},
	x tick label style={rotate=45,anchor=east, font=\scriptsize},
	xtick=data,
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=50, ymax=60,
	ytick={50,55,60},
	legend pos=north west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	
	\addplot[
	color=black,
	mark=x,
	]
	coordinates {
		([500*2],55.0)([500*3],54.4)([500*4],53.4)([800*2],54.9)([800*3],54.3)([800*4],53.4)([1000*2],55.1)([1000*3],54.3)([1000*4],53.7)
	};
	
	\addplot[
	color=black,
	mark=square,
	]
	coordinates {
		([500*2],54.0)([500*3],53.0)([500*4],52.4)([800*2],53.8)([800*3],53.4)([800*4],52.3)([1000*2],54.0)([1000*3],53.0)([1000*4],52.7)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{axis}[
	title={DBN-JKU-6seg-ch SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={[500*2],[500*3],[500*4],[800*2],[800*3],[800*4],[1000*2],[1000*3],[1000*4]},
	x tick label style={rotate=45,anchor=east, font=\scriptsize},
	xtick=data,
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=45, ymax=55,
	ytick={45,50,55},
	legend pos=north west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	
	\addplot[
	color=black,
	mark=x,
	]
	coordinates {
		([500*2],50.8)([500*3],50.8)([500*4],50.5)([800*2],50.9)([800*3],50.6)([800*4],50.5)([1000*2],50.8)([1000*3],50.9)([1000*4],50.5)
	};
	
	\addplot[
	color=black,
	mark=square,
	]
	coordinates {
		([500*2],50.4)([500*3],50.2)([500*4],50.3)([800*2],50.5)([800*3],50.2)([800*4],50.1)([1000*2],50.3)([1000*3],50.5)([1000*4],50.2)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\caption{Exploring different network configurations at -ch level. All models are trained with JKU-6seg-ch.}
	\label{fig:dbn-ch-configs}
\end{figure}

\Hsection{-ns level}

\begin{figure}[htb]
	\centering
	\begin{tikzpicture}
	\begin{axis}[
	title={FCNN-JKU-6seg-ns SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={[500*2],[500*3],[500*4],[800*2],[800*3],[800*4],[1000*2],[1000*3],[1000*4]},
	x tick label style={rotate=45,anchor=east, font=\scriptsize},
	xtick=data,
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=40, ymax=70,
	ytick={40,50,60,70},
	legend pos=north west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	\addplot[
	color=black,
	mark=x,
	]
	coordinates {
		([500*2],52.4)([500*3],52.5)([500*4],52.3)([800*2],52.7)([800*3],52.6)([800*4],52.6)([1000*2],52.8)([1000*3],52.9)([1000*4],52.9)
	};
	
	\addplot[
	color=black,
	mark=square,
	]
	coordinates {
		([500*2],50.0)([500*3],49.6)([500*4],49.6)([800*2],49.7)([800*3],49.4)([800*4],49.1)([1000*2],49.2)([1000*3],49.5)([1000*4],49.8)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{axis}[
	title={DBN-JKU-6seg-ns SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={[500*2],[500*3],[500*4],[800*2],[800*3],[800*4],[1000*2],[1000*3],[1000*4]},
	x tick label style={rotate=45,anchor=east, font=\scriptsize},
	xtick=data,
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=40, ymax=70,
	ytick={40,50,60,70},
	legend pos=north west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	\addplot[
	color=black,
	mark=x,
	]
	coordinates {
		([500*2],54.5)([500*3],54.6)([500*4],54.4)([800*2],54.5)([800*3],54.7)([800*4],53.0)([1000*2],54.4)([1000*3],53.8)([1000*4],51.6)
	};
	
	\addplot[
	color=black,
	mark=square,
	]
	coordinates {
		([500*2],53.0)([500*3],53.0)([500*4],52.8)([800*2],52.9)([800*3],53.0)([800*4],51.3)([1000*2],52.7)([1000*3],52.3)([1000*4],50.1)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\caption{Exploring different network configurations at -ns level. All models are trained with JKU-6seg-ns.}
	\label{fig:dbn-ns-configs}
\end{figure}


\subsection{Segment tiling} \label{sec:3-p3}

\Hsection{-ch level}

\pgfplotsset{width=8cm,height=4cm,every node near coord/.append style={font=\scriptsize}}
\begin{figure}[htb]
	\centering
	\begin{tikzpicture}
	\begin{axis}[
	title={FCNN-JKU-ch-[800*2] SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={1,2,3,6,9,12},
	x tick label style={font=\scriptsize},
	xtick=data,
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=40, ymax=70,
	ytick={40,50,60,70},
	legend pos=south west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	\addplot[ % Training
	color=black,
	mark=x,
	]
	coordinates {
		(1,54.9)(2,55.3)(3,55.2)(6,54.9)(9,54.6)(12,54.4)
	};
	
	\addplot[ % validation
	color=black,
	mark=square,
	]
	coordinates {
		(1,54.5)(2,54.6)(3,54.5)(6,53.8)(9,54.0)(12,53.4)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{axis}[
	title={DBN-JKU-ch-[800*2] SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={1,2,3,6,9,12},
	x tick label style={font=\scriptsize},
	xtick=data,
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=40, ymax=70,
	ytick={40,50,60,70},
	legend pos=south west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	\addplot[ % Training
	color=black,
	mark=x,
	]
	coordinates {
		(1,50.1)(2,50.6)(3,50.5)(6,50.9)(9,52.4)(12,56.1)
	};
	
	\addplot[ % validation
	color=black,
	mark=square,
	]
	coordinates {
		(1,49.7)(2,50.2)(3,50.2)(6,50.5)(9,51.7)(12,55.7)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{axis}[
	title={BLSTM-RNN-JKU-ch-[800*2] SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={1,2,3,6,9,12},
	x tick label style={font=\scriptsize},
	xtick=data,
	xlabel={number of frames in segment tiling},
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=40, ymax=70,
	ytick={40,50,60,70},
	legend pos=south west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	\addplot[ % Training
	color=black,
	mark=x,
	]
	coordinates {
		(1,56.3)(2,57.9)(3,59.0)(6,58.7)(9,58.9)(12,58.6)
	};
	
	\addplot[ % validation
	color=black,
	mark=square,
	]
	coordinates {
		(1,54.8)(2,56.2)(3,57.2)(6,56.7)(9,56.8)(12,56.4)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\caption{Exploring effect of segment tiling at -ch level. All models are trained with JKU-ch-[800*2]}
	\label{fig:N-frame}
\end{figure}

\Hsection{-ns level}

\pgfplotsset{width=8cm,height=4cm,every node near coord/.append style={font=\scriptsize}}
\begin{figure}[htb]
	\centering
	\begin{tikzpicture}
	\begin{axis}[
	title={FCNN-JKU-ns-[800*2] SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={1,2,3,6,9,12},
	x tick label style={font=\scriptsize},
	xtick=data,
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=40, ymax=70,
	ytick={40,50,60,70},
	legend pos=north west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	\addplot[ % Training
	color=black,
	mark=x,
	]
	coordinates {
		(1,53.0)(2,53.2)(3,53.1)(6,52.7)(9,51.6)(12,52.1)
	};
	
	\addplot[ % validation
	color=black,
	mark=square,
	]
	coordinates {
		(1,50.8)(2,50.1)(3,50.3)(6,49.7)(9,49.0)(12,48.9)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{axis}[
	title={DBN-JKU-ns-[800*2] SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={1,2,3,6,9,12},
	x tick label style={font=\scriptsize},
	xtick=data,
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=40, ymax=70,
	ytick={40,50,60,70},
	legend pos=north west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	\addplot[ % Training
	color=black,
	mark=x,
	]
	coordinates {
		(1,49.8)(2,54.2)(3,54.2)(6,54.5)(9,54.0)(12,54.0)
	};
	
	\addplot[ % validation
	color=black,
	mark=square,
	]
	coordinates {
		(1,49.2)(2,53.1)(3,53.2)(6,52.9)(9,52.6)(12,52.6)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\begin{tikzpicture}
	\begin{axis}[
	title={BLSTM-RNN-JKU-ns-[800*2] SeventhsBass Performances},
	title style = {font=\scriptsize},
	x label style={font=\scriptsize},
	symbolic x coords={1,2,3,6,9,12},
	x tick label style={font=\scriptsize},
	xtick=data,
	xlabel={number of frames in segment tiling},
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	ymin=50, ymax=80,
	ytick={50,60,70,80},
	legend pos=north west,
	legend style={legend columns=-1, font=\scriptsize},
	ymajorgrids=true,
	grid style=dashed,
	]
	\addplot[ % Training
	color=black,
	mark=x,
	]
	coordinates {
		(1,60.4)(2,61.6)(3,64.0)(6,63.4)(9,63.0)(12,62.3)
	};
	
	\addplot[ % validation
	color=black,
	mark=square,
	]
	coordinates {
		(1,53.7)(2,54.0)(3,54.9)(6,54.9)(9,54.5)(12,54.9)
	};
	\legend{Training, Validation} 
	\end{axis}
	\end{tikzpicture}
	\caption{Exploring effect of segment tiling at -ns level. All models are trained with JKU-ns-[800*2]}
	\label{fig:N-frame-ns}
\end{figure}

\subsection{Training data size}\label{sec:3-p5}

\Hsection{-ch level}

\begin{figure}[htb]
	\centering
	\pgfplotsset{width=8cm,height=4cm,every node near coord/.append style={font=\scriptsize}}
	\subfigure{
		\begin{tikzpicture}
		\begin{axis}[
		title={SeventhsBass Performances within FCNN-6seg-ch-[800*2]},
		title style = {font=\scriptsize},
		x label style={font=\scriptsize},
		symbolic x coords={JK,JKU,JKUR,JKURB},
		x tick label style={font=\scriptsize},
		xtick=data,
		ylabel={WCSR $\times$ 100},
		y label style={font=\scriptsize},
		ymin=30, ymax=60,
		ytick={30,40,50,60},
		legend pos=south east,
		legend style={legend columns=-1, font=\scriptsize},
		ymajorgrids=true,
		grid style=dashed,
		]
		\addplot[ % Training
		color=black,
		mark=x,
		]
		coordinates {(JK,41.7)(JKU,54.9)(JKUR,58.4)(JKURB,56.3)};
		
		\addplot[ % validation
		color=black,
		mark=square,
		]
		coordinates {(JK,39.7)(JKU,53.8)(JKUR,57.6)(JKURB,55.5)};
		\legend{Training, Validation} 
		\end{axis}
		\end{tikzpicture}
	}
	\subfigure{
		\begin{tikzpicture}
		\begin{axis}[
		title={SeventhsBass Performances within DBN-6seg-ch-[800*2]},
		title style = {font=\scriptsize},
		x label style={font=\scriptsize},
		symbolic x coords={JK,JKU,JKUR,JKURB},
		x tick label style={font=\scriptsize},
		xtick=data,
		ylabel={WCSR $\times$ 100},
		y label style={font=\scriptsize},
		ymin=30, ymax=60,
		ytick={30,40,50,60},
		legend pos=south east,
		legend style={legend columns=-1, font=\scriptsize},
		ymajorgrids=true,
		grid style=dashed,
		]
		\addplot[ % Training
		color=black,
		mark=x,
		]
		coordinates {(JK,34.8)(JKU,50.9)(JKUR,56.2)(JKURB,55.4)};
		
		\addplot[ % validation
		color=black,
		mark=square,
		]
		coordinates {(JK,35.7)(JKU,50.5)(JKUR,56.2)(JKURB,55.0)};
		\legend{Training, Validation} 
		\end{axis}
		\end{tikzpicture}
	}
	\subfigure{
		\begin{tikzpicture}
		\begin{axis}[
		title={SeventhsBass Performances within BLSTM-RNN-6seg-ch-[800*2]},
		title style = {font=\scriptsize},
		x label style={font=\scriptsize},
		symbolic x coords={JK,JKU,JKUR,JKURB},
		x tick label style={font=\scriptsize},
		xtick=data,
		ylabel={WCSR $\times$ 100},
		y label style={font=\scriptsize},
		ymin=50, ymax=70,
		ytick={50,60,70},
		legend pos=north west,
		legend style={legend columns=-1, font=\scriptsize},
		ymajorgrids=true,
		grid style=dashed,
		]
		\addplot[ % Training
		color=black,
		mark=x,
		]
		coordinates {(JK,58.2)(JKU,58.7)(JKUR,61.7)(JKURB,61.2)};
		
		\addplot[ % validation
		color=black,
		mark=square,
		]
		coordinates {(JK,54.7)(JKU,56.7)(JKUR,59.2)(JKURB,59.7)};
		\legend{Training, Validation} 
		\end{axis}
		\end{tikzpicture}
	}
	\caption{Exploring different training data size at -ch level. All models are trained with 6seg-ch-[800*2].}
	\label{fig:ch-data}
\end{figure}

\Hsection{-ns level}

\begin{figure}[htb]
	\centering
	\pgfplotsset{width=8cm,height=4cm,every node near coord/.append style={font=\scriptsize}}
	\subfigure{
		\begin{tikzpicture}
		\begin{axis}[
		title={SeventhsBass Performances within FCNN-6seg-ns-[800*2]},
		title style = {font=\scriptsize},
		%xlabel={Network Configuration},
		x label style={font=\scriptsize},
		symbolic x coords={JK,JKU,JKUR,JKURB},
		x tick label style={font=\scriptsize},
		xtick=data,
		ylabel={WCSR $\times$ 100},
		y label style={font=\scriptsize},
		ymin=40, ymax=60,
		ytick={40,50,60},
		legend pos=south east,
		legend style={legend columns=-1, font=\scriptsize},
		ymajorgrids=true,
		grid style=dashed,
		]
		\addplot[ % Training
		color=black,
		mark=x,
		]
		coordinates {(JK,48.4)(JKU,52.7)(JKUR,56.7)(JKURB,57.5)};
		
		\addplot[ % validation
		color=black,
		mark=square,
		]
		coordinates {(JK,44.9)(JKU,49.7)(JKUR,52.9)(JKURB,49.9)};
		\legend{Training, Validation} 
		\end{axis}
		\end{tikzpicture}
	}
	\subfigure{
		\begin{tikzpicture}
		\begin{axis}[
		title={SeventhsBass Performances within DBN-6seg-ns-[800*2]},
		title style = {font=\scriptsize},
		%xlabel={Network Configuration},
		x label style={font=\scriptsize},
		symbolic x coords={JK,JKU,JKUR,JKURB},
		x tick label style={font=\scriptsize},
		xtick=data,
		ylabel={WCSR $\times$ 100},
		y label style={font=\scriptsize},
		ymin=30, ymax=60,
		ytick={30,40,50,60},
		legend pos=south east,
		legend style={legend columns=-1, font=\scriptsize},
		ymajorgrids=true,
		grid style=dashed,
		]
		\addplot[ % Training
		color=black,
		mark=x,
		]
		coordinates {(JK,33.2)(JKU,54.5)(JKUR,55.9)(JKURB,55.4)};
		
		\addplot[ % validation
		color=black,
		mark=square,
		]
		coordinates {(JK,32.6)(JKU,52.9)(JKUR,54.6)(JKURB,54.2)};
		\legend{Training, Validation} 
		\end{axis}
		\end{tikzpicture}
	}
	\subfigure{
		\begin{tikzpicture}
		\begin{axis}[
		title={SeventhsBass Performances within BLSTM-RNN-6seg-ns-[800*2]},
		title style = {font=\scriptsize},
		x label style={font=\scriptsize},
		symbolic x coords={JK,JKU,JKUR,JKURB},
		x tick label style={font=\scriptsize},
		xtick=data,
		ylabel={WCSR $\times$ 100},
		y label style={font=\scriptsize},
		ymin=50, ymax=70,
		ytick={50,60,70},
		legend pos=north west,
		legend style={legend columns=-1, font=\scriptsize},
		ymajorgrids=true,
		grid style=dashed,
		]
		\addplot[ % Training
		color=black,
		mark=x,
		]
		coordinates {(JK,60.6)(JKU,63.4)(JKUR,63.3)(JKURB,64.2)};
		
		\addplot[ % validation
		color=black,
		mark=square,
		]
		coordinates {(JK,50.7)(JKU,54.9)(JKUR,56.9)(JKURB,58.4)};
		\legend{Training, Validation} 
		\end{axis}
		\end{tikzpicture}
	}
	\caption{Exploring training data size at -ns level. All models are trained with 6seg-ns-[800*2].}
	\label{fig:ns-data}
\end{figure}

\begin{figure*}[htb]
	\centering
	\pgfplotsset{width=18cm,height=4cm,every node near coord/.append style={font=\scriptsize}}
	\begin{tikzpicture}
	\begin{axis}[
	title={Average per chord WCSRs from all 6seg-[800*2] models},
	title style = {font=\scriptsize},
	ybar=3pt,
	bar width=5pt,
	enlargelimits=0.15,
	legend style={at={(0.5,-0.4)},
		anchor=north,legend columns=-1},
	ylabel={WCSR $\times$ 100},
	y label style={font=\scriptsize},
	symbolic x coords={maj, min, maj/3, maj/5, maj7, dom7, min/b3, min/5, min7, 7/b7},
	x tick label style={rotate=30,anchor=east, font=\scriptsize},
	xtick=data,
	ymin=10, ymax=75,
	%nodes near coords,
	nodes near coords align={vertical},
	legend style={font=\scriptsize},
	]
	\addplot [ybar,fill=white,draw=black] coordinates {(maj,72.6)(min,49.8)(maj/3,26.6)(maj/5,13.5)(maj7,13.0)(dom7,7.5)(min/b3,3.6)(min/5,5.3)(min7,32.9)(7/b7,23.7)};
	
	\addplot [ybar,fill=brown,draw=black] coordinates {(maj,74.0)(min,47.5)(maj/3,22.6)(maj/5,6.7)(maj7,4.8)(dom7,5.1)(min/b3,0)(min/5,0)(min7,25.0)(7/b7,0.1)};
	
	\addplot [ybar,fill=black,draw=black] coordinates {(maj,71.9)(min,56.9)(maj/3,49.9)(maj/5,27.8)(maj7,38.1)(dom7,23.9)(min/b3,15.1)(min/5,17.9)(min7,46.0)(7/b7,43.2)};
	
	\legend{FCNN,DBN,BLSTM-RNN}
	\end{axis}
	\end{tikzpicture}
	\caption{Performance on different chords in different neural nets. All models are trained with 6seg-[800*2].}
	\label{fig:skewed}
\end{figure*}
